SciNav: A General Agent Framework for Scientific Coding Tasks

Autonomous science agents built on large language models (LLMs) are increasingly used to generate hypotheses, design experiments, and produce reports. However, prior work mainly targets open-ended scientific problems with subjective outputs that are difficult to evaluate. Scientific coding benchmarks, by contrast, provide executable outputs for objective assessment. Existing approaches remain engineering-driven pipelines, revealing the need for structured, end-to-end science agent frameworks for scientific coding tasks. We address this gap by focusing on scientific coding tasks, where evaluation can be made rigorously, and introducing an agent framework SciNav (Scientific Navigator) that enables more effective solution exploration. Our framework is designed to operate under constrained search budgets, moving beyond reliance on pre-defined success metrics and prolonged search cycles. Inspired by findings that comparative judgments often reveal finer-grained quality differences and therefore provide greater discriminative power than absolute scoring, our framework leverages pairwise relative judgments within a tree search process to select top-K promising solution branches, prune low-potential ones, and progressively narrow down the solution candidates on the selected branches guided by relative comparisons. We demonstrate our agent's effectiveness across different types of tasks on two benchmarks. Experiments show that SciNav significantly outperforms direct prompting and prior agents like OpenHands and Self-Debug across different base models, task types, and difficulty levels, and exceeds different frontier comparators such as random selection and LLM absolute scoring. These results confirm the strength of our agent design and highlight the effectiveness of relative judgment-guided top-K search for high-quality scientific coding, marking a step toward more practical science agents.

==> algo/elo_tree_search.tex <==
\begin{algorithm}[H]
\caption{Elo-Tree Search (ETS)}
\label{alg:ets}
\KwIn{
    Task description $T$, 
    Search depth $d_{\max}$, 
    Branching factor $b$, 
    Elo parameters $(K, R_0)$
}
\KwOut{
    Best solution $s^\ast$
}

\BlankLine
Initialize root node $n_0$ with empty solution and Elo rating $R_0$\;
Initialize priority queue $Q \leftarrow \{n_0\}$\;

\While{$Q$ not empty}{
    Pop node $n$ with highest priority from $Q$\;
    \If{$\text{depth}(n) \ge d_{\max}$}{
        \Continue\;
    }
    
    Generate $b$ candidate child nodes $\{c_1, \dots, c_b\}$ from $n$\;
    
    \ForEach{pair $(c_i, c_j)$ in tournament schedule}{
        $winner \leftarrow \text{LLM\_Judge}(T, c_i, c_j)$\;
        Update Elo ratings $R_{c_i}, R_{c_j}$ using $K$ and match result\;
    }
    
    Insert all children into $Q$ with priority $\propto R_{c_k}$\;
}

$s^\ast \leftarrow$ solution with highest Elo rating among all explored nodes\;
\Return $s^\ast$\;
\end{algorithm}



% \begin{algorithm}[H]
% \caption{Elo-Tree Search (ETS)}
% \label{alg:ets}
% \begin{algorithmic}[1] % [1] adds line numbers
% \State \textbf{Input:} Task description $T$, Search depth $d_{\max}$, Branching factor $b$, Elo parameters $(K, R_0)$
% \State \textbf{Output:} Best solution $s^\ast$
% \Statex

% \State Initialize root node $n_0$ with empty solution and Elo rating $R_0$
% \State Initialize priority queue $Q \gets \{n_0\}$

% \While{$Q$ not empty}
%     \State Pop node $n$ with highest priority from $Q$
%     \If{$\text{depth}(n) \ge d_{\max}$}
%         \State \textbf{continue}
%     \EndIf
    
%     \State Generate $b$ candidate child nodes $\{c_1, \dots, c_b\}$ from $n$
    
%     \ForAll{pair $(c_i, c_j)$ in tournament schedule}
%         \State $winner \gets \text{LLM\_Judge}(T, c_i, c_j)$
%         \State Update Elo ratings $R_{c_i}, R_{c_j}$ using $K$ and match result
%     \EndFor
    
%     \State Insert all children into $Q$ with priority $\propto R_{c_k}$
% \EndWhile

% \State $s^\ast \gets$ solution with highest Elo rating among all explored nodes
% \State \Return $s^\ast$
% \end{algorithmic}
% \end{algorithm}



==> algo/pairwise_tree_search.tex <==
\begin{algorithm}[t]
\caption{PRESTO: Pairwise-Ranked Best-First Tree Search}
\label{alg:presto}
\begin{algorithmic}[1]
\Require Task description $T$, initial candidates $S_0$, comparison budget $B$, expansion limit $L$
\State Initialize priority queue $\mathcal{Q} \gets S_0$ \Comment{Store nodes with Elo rating}
\State Initialize Elo ratings $R(s) \gets R_0$ for all $s \in S_0$
\While{$\mathcal{Q}$ not empty and budget $B > 0$}
    \State $C \gets$ \textsc{SampleCandidates}($\mathcal{Q}, k$) \Comment{Select $k$ candidates to compare}
    \For{each unordered pair $(s_i, s_j) \in C$}
        \State $w \gets$ \textsc{LLMCompare}($T, s_i, s_j$) \Comment{Ask LLM which is better}
        \State Update $R(s_i), R(s_j)$ using Elo update with winner $w$
        \State $B \gets B - 1$
    \EndFor
    \State $s^\ast \gets \arg\max_{s \in \mathcal{Q}} R(s)$ \Comment{Best candidate so far}
    \If{\textsc{StoppingCriterion}($s^\ast$)}
        \State \Return $s^\ast$ \Comment{Terminate if solution is good enough}
    \EndIf
    \State $E \gets$ \textsc{ExpandNode}($s^\ast$, limit $L$) \Comment{Generate $L$ new solutions from $s^\ast$}
    \For{each $e \in E$}
        \State Add $e$ to $\mathcal{Q}$ with initial Elo rating $R_0$
    \EndFor
    \State Remove $s^\ast$ from $\mathcal{Q}$ \Comment{Do not expand again}
\EndWhile
\State \Return $\arg\max_{s \in \mathcal{Q}} R(s)$ \Comment{Best candidate found}
\end{algorithmic}
\end{algorithm}


==> comparison_with_existing_agents.tex <==
\section{Comparison with Existing Science Agents}

To situate our work, we compare existing science agents along their scope, planning mechanisms, retrieval usage, evaluation strategies, and target artifacts. As shown in Table~\ref{tab:science_agents_comparison}, prior systems largely operate in a full-cycle, open-ended setting, aiming to cover the entire research pipeline that produces outputs such as hypotheses, experiments, or reports, which resist systematic automatic evaluation. Others focus on narrower domains (e.g., machine learning coding tasks) and primarily rely on task-defined metrics that assume well-specified success criteria. In contrast, our proposed agent, \texttt{SciNav}, is designed for scientific coding tasks with executable outputs, enabling principled evaluation. This distinction motivates our framework, which introduces relative-judgment–guided tree search to efficiently explore solution spaces under realistic computational budgets.

==> figures/k_plot.tex <==
\begin{figure}[htbp]
\begin{center}
%\framebox[4.0in]{$\;$}
% \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\includegraphics[width=0.8\linewidth]{figures/k_plot.png}
\end{center}
\vspace{-6mm}  % <-- adjust this value as needed
\caption{\textcolor{revision}{Average score across different values of 
$K \in \{1,2,3,4,5\}$ in a preliminary study on 30 randomly sampled DA-Code tasks. $K=2$ achieves the highest average performance, and is therefore used for all subsequent experiments.}}
\label{fig:k_plot}
\end{figure}



==> figures/k_plot_cost.tex <==
\begin{figure}[htbp]
\begin{center}
%\framebox[4.0in]{$\;$}
% \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\includegraphics[width=0.8\linewidth]{figures/k_plot_cost.png}
\end{center}
\vspace{-6mm}  % <-- adjust this value as needed
\caption{\textcolor{revision}{Agent cost across different values of 
$K \in \{1,2,3,4,5\}$.}}
\label{fig:k_plot_cost}
\end{figure}



==> figures/overview.tex <==
\begin{figure*}[t]
\begin{center}
%\framebox[4.0in]{$\;$}
% \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\includegraphics[width=0.99\linewidth]{figures/overview.png}
\end{center}
\caption{An overview of our agent framework: \texttt{SciNav}.}
\label{fig:overview}
\end{figure*}

==> figures/tree_search.tex <==
\begin{figure*}[t]
\begin{center}
%\framebox[4.0in]{$\;$}
% \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\includegraphics[width=0.99\linewidth]{figures/elo_rating_verifier_final.png}
\end{center}
\caption{An overview of Elo Rating verifier in tree search.}
\label{fig:tree_search}
\end{figure*}

==> limitation.tex <==
\section*{Limitations}

One limitation of our current framework is that it requires generating an entire code block in a single step, without support for incremental synthesis or partial execution feedback. As a result, for tasks that demand generating very long programs which are beyond the model's capacity, our agent may become unsuitable for effectively handling such cases. Additionally, once the agent enters the self-improvement stage, it lacks the ability to autonomously determine when to stop; instead, it continues until the predefined maximum number of total steps is reached. This rigid stopping criterion can result in unnecessary computation or missing a high-quality solution that has already been found earlier\nop{missed opportunities for early convergence when a high-quality solution has already been found}.

==> prompts.tex <==
% \begin{center}
%     {\huge General Comments} \\
% \end{center}


% {\large
% 1. We have addressed the great majority of the suggestions from the reviewers. Only a few
% suggestions that could not be addressed have been properly justified;\\

% 2. We have performed more experiments encompassing a new dataset;\\

% 3. We have performed more experiments to present the sensitivity analysis of the
% parameters employed by our approach; \\

% 4. Following the suggestions of the reviewers, we have improved many sections of the article
% by pointing out other related works, adding new examples, discussing the results in more
% details and presenting lessons learned from the obtained experimental results; \\

% 5. We have highlighted in blue the sentences and results added to the new version of our
% manuscript; \\

% 6. We would like to extend our sincere gratitude for the detailed and constructive feedback
% provided on our manuscript. Your insights and suggestions have been invaluable and have
% significantly contributed to improving the quality and clarity of our work. The following tables
% list these suggestions in addition to the respective justifications or solutions implemented. \\
% }


\begin{figure*}[htbp]
\begin{tcolorbox}
[colback=white, colframe=gray!60!black,
title={\huge Reviewer 1 - Page 1}, fontupper=\footnotesize, fonttitle=\footnotesize]
{\Large

We mark the relevant revision part in the paper using \textcolor{reviewer1}{red color for reviewer 1}. Note execution accuracy results are marked as \textcolor{reviewer3}{green} in Table \ref{tab:bird_exec_acc}.\\

\textbf{\#\#\# Suggestion}: \\

The paper should be compared to the following paper, which also studied the problem of schema evolution and provided a benchmark dataset on real queries where both the train and the test data reflect schema changes:

[1] Jonathan Fürst, Catherine Kosten, Farhad Nooralahzadeh, Yi Zhang, Kurt Stockinger: Evaluating the Data Model Robustness of Text-to-SQL Systems Based on Real User Queries. EDBT 2025: 158-170 \\

\textbf{\#\#\# Response}: \\

We compare our work with theirs from the following four perspectives: \\
(1) Motivation: 

[1] explores three manually designed schema versions for a single Football database, aiming to identify a schema that is beneficial for SQL writing. Their first evolution (v1 → v2) addresses 1:N foreign key mappings, which can complicate pre-/post-processing in some text-to-SQL models. However, this also increases the number of tables and required joins. So their second evolution (v2 → v3) is to reduce the JOIN complexity. In contrast, our work takes a different view of schema evolution. Schema evolution is driven not only by structural reorganization (e.g., splitting or merging tables), but also by the need to incorporate new information (e.g., adding columns or tables), and we analyze how these changes affect NL2SQL performance.
% In contrast, our work focuses on schema evolution more broadly, motivated by practical needs not only for schema reorganization such as splitting and merging tables, but also considering how new information required the scheme change such as adding columns or tables, and investigates how such changes impact NL2SQL performance.

(2) Schema Evolution Types:

While [1] focuses primarily on reducing PK/FK references and minimizing JOIN complexity, our work explores the schema evolution from a different angle, where we introduce a more comprehensive and systematic taxonomy of schema evolution types. We analyze both table-level and column-level changes, including adding, removing, renaming, splitting, and merging columns and tables and aim at offering a broader and more structured exploration of schema evolution.

(3) Model Scope:

[1] includes earlier models like ValueNet and PICARD, which rely on pre- and post-processing. We mainly evaluate more recent and powerful LLMs, including fine-tuning advanced open-source models (CodeLlama, Mistral, SQLCoder, LLaMA 3) and prompting closed-source models (GPT-3.5, GPT-4). These recent models can be used without preprocessing or postprocessing steps for SQL generation and are still under-explored. 

(4) Data Scale and Generalizability:

[1] evaluates on three manually curated schema versions of a single Football database. In contrast, our work builds on BIRD, a complex, realistic multi-database benchmark. Our framework enables systematic schema evolution across multiple databases, providing more scalable and generalizable experimental results. This directly addresses a limitation in [1], which is confined to a single-domain, single-database setting. \\


% (1) From the motivataion perspective, their work explores three versions of designed schema for their proposed Football database and tries to find a better database schema design that is beneficial for SQL writing. For their first evolution from design v1 to design v2, the motivation of this evolution is to address the 1:N foreign key mappings between tables, which will cause issues during the pre-processing or post-processing stage for several text-to-SQL models. From design v1 to design v2, there are more tables in the database, and the SQL query needs to join more tables. Our work focuses on scheme evolution, which not only covers database schema reorganization, but inspired by when new information come will need us to revise the existing database design such as add columns, add tables. and want to explore how these change will affect the NL2SQL performance. \\
% (2) From the scheme evolution types perspective, [1] mainly revise their schema design to reduce PK/FK references among tables and reduce JOIN paths for SQL queries. while our work mainly try to give a more comprehensive, systematic and structured taxonomy and analysis for different schema evolution types. Instead of just analyzing these two specific types, we systematically build a taxonomy to explore the table-level and column-level schema evolution that covers more comprehensive types such as adding/removing/renaming/splitting/merging tables and columns. \\
% (3) From the model perspective, we mainly explore the more advanced open-sourced models (codellama, mistral, sqlcoder and llama3) and closed-sourced models (gpt-3.5 and gpt-4). The ValueNet and Picard in their work are relatively older models that still require pre-processing and post-processing steps. As the more advanced open-sourced models have emerged recently and are much more powerful than the models selected by [1], we consider that our selected advanced models are still under-explored for this schema evolution problem and are more convenient which don’t require pre-processing and post-processing. \\
% (4) From the data scale perspective, [1] only three manually designed versions of the schema and the schema is within the same database. Our work builds our dataset based on a complex, realistic and multiple-database dataset: BIRD. We provide the framework that allows us to systematically get different versions of the schema under more comprehensive schema evolution types and apply it on different databases in BIRD instead of just a single Football database. So our analysis is based on multiple databases and provides more reliable quantitative results and our findings will be more generalizable, which can address the limitation mentioned in [1], that they only do experiments on a single database dataset. \\

\textbf{\#\#\# Revised Section}: \\

We add this work into Table \ref{tab:comparison_with_existing_benchmarks} to compare with other schema perturbation related work: DrSpider, ADVETA, MT-TEQL and our EvoSchema. Besides, we also revise the Section \ref{related_work} (Related Work) and Section \ref{comparison_with_existing_benchmarks} (Comparison with Existing Benchmarks) to compare this work.

% \noindent\rule{\linewidth}{0.5pt}

}
\end{tcolorbox}
% \caption{\textbf{Schema augmentation} task. This task is to populate the possible headers for a table, given the table caption and the seed table header.}
% \label{fig:schema_aug}
\end{figure*}


\begin{figure*}[htbp]
\begin{tcolorbox}
[colback=white, colframe=gray!60!black,
title={\huge Reviewer 1 - Page 2}, fontupper=\footnotesize, fonttitle=\footnotesize]
{\Large

We mark the relevant revision part in the paper using \textcolor{reviewer1}{red color for reviewer 1}. Note execution accuracy results are marked as \textcolor{reviewer3}{green} in Table \ref{tab:bird_exec_acc}.\\\

\textbf{\#\#\# Suggestion}: \\

In general, the experiments need to be better described and be modelled in a more realistic setting where both the schema and the queries evolve over time. It is unrealistic that the schema evolves over time and the testing is done on non-evolved schema. In other words, the test set queries should be extended with new queries against evolved schema. \\

\textbf{\#\#\# Response}: \\

We want to clarify that the reviewer misunderstood our experiment design. We indeed adopted the reviewer-mentioned realistic setting and designed the experiment to let both the schema and SQL queries evolve over time. And for both training data and test data, we included new schema and new queries against evolved schema. As the second paragraph (Schema Perturbations) in Section \ref{seed_data_select} (Seed Dataset Selection) in the paper mentioned, we apply the schema evolution on the entire BIRD dataset and get both the new schema and new SQL queries. The train/test split examples are aligned with the original BIRD train/dev split. Table~\ref{tab:data_stat_plus_manipulated_stat} presents the data statistics used in our experiments. ``Original'' refers to the raw BIRD training and evaluation data without any schema evolution. While other rows show each schema evolution type, and we report the corresponding training and evaluation statistics. Here, ``eval" denotes the test set, which includes both evolved schemas and new queries. In Table \ref{tab:bird_main_results2}, the row labeled ``Original" reports performance on the original BIRD test set (no schema evolution), while the other rows (e.g., add columns) show results on test sets where both the schema and queries have been modified. For each model (e.g., CodeLlama, Mistral, Llama3 and SQLCoder), there are two columns to show the results. w/o column indicates the model is trained without perturbation training data, while w/ column indicates the model is trained with perturbation data. For both trained w/o and w/ perturbation training data, we evaluate them on non-evolved (Original) test set and each type of evolved test set.  \\


\textbf{\#\#\# Highlighted Section}: \\

We highlight how we prepare our train/eval data for both non-evolved and evolved sets. Please check `Schema Perturbations' in Section \ref{seed_data_select} (Seed Dataset Selection) in the paper.

Please check Table \ref{tab:bird_main_results2} and Table \ref{tab:bird_exec_acc} for results on both the non-evolved test set and evolved test set. Note: for each model (e.g., CodeLlama, etc), w/o column indicates the model is trained without perturbation train data, while w/ column indicates the model is trained with perturbation train data. For both trained w/o and w/ perturbation train data, we evaluate them on non-evolved (Original) test set and each type of evolved test set. \\

\noindent\rule{\linewidth}{0.5pt}

\textbf{\#\#\# Suggestion}: \\

It seems that the test data is the same whereas the training used is without and with perturbations. It would be important to add new test queries that are executed against the schema that evolved over time. \\

\textbf{\#\#\# Response}: \\

As mentioned above, our test setting includes both non-evolved and evolved queries. The non-evolved queries come from the original BIRD dev set, while the evolved queries are generated by applying ten schema evolution types to the original BIRD dev set. Similarly, the training set includes both the original (non-evolved) BIRD training data and the corresponding evolved versions.\\




}
\end{tcolorbox}
\end{figure*}


\begin{figure*}[htbp]
\begin{tcolorbox}
[colback=white, colframe=gray!60!black,
title={\huge Reviewer 1 - Page 3}, fontupper=\footnotesize, fonttitle=\footnotesize]
{\Large

We mark the relevant revision part in the paper using \textcolor{reviewer1}{red color for reviewer 1}. Note execution accuracy results are marked as \textcolor{reviewer3}{green} in Table \ref{tab:bird_exec_acc}.\\\

\textbf{\#\#\# Suggestion}: \\

The evaluation needs to be improved. Table 3 shows the F1 score of table match for various LLMs but no execution accuracy. Table 4 only shows execution accuracy, but it is not clear for which LLM. \\

\textbf{\#\#\# Response and Revised Section}: \\


We add Table \ref{tab:bird_exec_acc} to show the execution accuracy for all the LLMs (CodeLlama, Mistral, Llama3, SQLCoder, GPT-3.5 and GPT4) mentioned in Table \ref{tab:bird_main_results2}. And also we add human evaluation results in Table \ref{tab:bird_human_eval}. \\


\noindent\rule{\linewidth}{0.5pt}

\textbf{\#\#\# Suggestion}: \\

The authors write “Since the NLQs are the same for adding or removing columns and tables”. This is not correct. When you remove columns and tables, existing NLQs might not work anymore. \\

\textbf{\#\#\# Response}: \\

When we apply removing columns and tables perturbations, we detect whether the gold SQL contains the columns or tables that will be removed. If yes, then the corresponding NLQs don't work, and we will change our ground truth for these NLQs as ``The table/column information is not enough for generating the SQL query to answer the question.'' We show our experiments in Section \ref{out_of_scope_exp} (Influence of Out-of-scope Types). If these removed tables and columns aren't included in the gold SQL, then these NLQs still work, and we can still examine how they will influence the SQL generation for these NLQs. \\


\noindent\rule{\linewidth}{0.5pt}

\textbf{\#\#\# Suggestion}: \\
The authors write “Add tables: We randomly add irrelevant tables to each question, and these tables are still in the same database as the relevant tables in BIRD. [..] The tables added don’t affect the NLQ and the gold SQL”. It is not clear why you want to add random tables in the SQL without affecting the NLQ. Can you give concrete example to 
justify this from a real-world perspective? \\


\textbf{\#\#\# Response}: \\


Thank you for your thoughtful question. Our goal in adding irrelevant tables is to simulate real-world scenarios where databases often contain many tables unrelated to a given user query. In such settings, a robust text-to-SQL model must be able to identify and focus on the relevant subset of the schema while ignoring distracting or unrelated tables.

For example, in a university database with tables such as Students, Courses, and Enrollments, a user may ask: “What are the names of students enrolled in CS101?” Although the correct SQL query only involves the three aforementioned tables, the full schema may also include tables like DormRooms or CafeteriaMenus, which are unrelated to the question. In this case, the model is expected to ignore these irrelevant tables and still generate the correct SQL. Our perturbation ``add tables'' intentionally mimics this setting by introducing such extraneous tables, without changing the NLQ or the gold SQL, in order to evaluate the model’s ability to remain focused and accurate in the presence of schema distraction.






}
\end{tcolorbox}
\end{figure*}



\begin{figure*}[htbp]
\begin{tcolorbox}
[colback=white, colframe=gray!60!black,
title={\huge Reviewer 1 - Page 4}, fontupper=\footnotesize, fonttitle=\footnotesize]
{\Large

We mark the relevant revision part in the paper using \textcolor{reviewer1}{red color for reviewer 1}. Note execution accuracy results are marked as \textcolor{reviewer3}{green} in Table \ref{tab:bird_exec_acc}.\\\

\textbf{\#\#\# Suggestion}: \\

When you split and merge tables, do you make sure that the properties of the three database normal forms are kept? \\


\textbf{\#\#\# Response}: \\

Thank you for the insightful question. While our primary focus is on simulating realistic schema evolution scenarios through table splits and merges, we take care to preserve the principles of the first three normal forms (1NF–3NF) as much as possible.

For table splitting, we ensure that: each resulting table maintains atomic values (1NF); non-key attributes depend on the full pimary key (2NF). And we avoid introducing transitive dependencies (3NF) by separating attributes that do not belong together functionally. For example, when splitting a table that combines student and course enrollment data, we create separate Students, Courses, and Enrollments tables, each with clearly defined primary keys and no redundant or derived attributes.

For table merging, we carefully monitor functional dependencies. But we admit that there is a risk that might introduce non-key to non-key dependencies unintentionally, especially when we merge too much descriptive data into one table. So there is a risk that it might violate 3NF.


 Overall, while our benchmark explores structural variations through schema evolution, we make an effort to preserve the principles of database normalization. \\



\noindent\rule{\linewidth}{0.5pt}



\textbf{\#\#\# Suggestion}: \\

The authors write “We randomly choose 200 generated examples to do manual review and reveal that GPT-3.5 demonstrates a strong understanding of the input context, effectively generating names that meet our requirement”. Can you quantify this better? What is the accuracy of these 200 queries? How do you evaluate the accuracy of other queries that are not manually verified? \\



\textbf{\#\#\# Response}: \\

Thank you for the question. We primarily use GPT-3.5 to rename column/table names or add new columns to the database schema. For SQL queries, we update the gold SQL by replacing original names with the GPT-3.5-generated ones based on the schema changes. So the key is to make sure GPT-3.5 can generate column names or table names correctly. To ensure name generation quality, we randomly sampled 200 examples and found that 94\% of them met our requirements. This automated approach is applied only to add columns, rename columns, and rename tables cases. For more complex schema evolution types, such as split and merge tables, manual verification is still required.

}
\end{tcolorbox}
\end{figure*}

% Thanks for the question. We mainly use GPT-3.5 to rename column/table names, or add column names into the database schema. For SQL queries, we will based on the schema name change to replace the original name in the gold SQL query to the new SQL query. So the key is to make sure GPT-3.5 can generate column names or table names correctly. We randomly select 200 examples and analyze whether the GPT-3.5 generated names meet our requirement. We found that there are 94\% examples can meet our requirements. We only do this for adding columns, renaming columns and renaming tables types. For other more complex schema evolution types like splitting or merging tables, we do need mannully verification.




==> prompts/llm_judge.tex <==
\begin{figure*}[t]
\begin{tcolorbox}
[colback=white, colframe=gray!60!black,
title={\Large LLM-Absolute Prompt}, fontupper=\footnotesize, fonttitle=\footnotesize]
{
Task description: \{\} \\
Response summary: \{\} \\
The generated code program is as following: \{program\}\\

Please generate a score between 0 to 100 to indicate how good and suitable the generated code matches the request. \\

You can have the explanation, reasoning or analysis, but please explicitly generate the score using the format **Score: **, e.g., **Score: 37** in your response.

}
\end{tcolorbox}
\end{figure*}
    

==> prompts/rubric_judge.tex <==
\begin{figure*}[t]
\begin{tcolorbox}
[colback=white, colframe=gray!60!black,
title={\Large Rubric-Absolute Prompt}, fontupper=\footnotesize, fonttitle=\footnotesize]
{
Task description: \{\} \\
Response summary: \{\} \\
The generated code program is as following: \{program\}\\
The grading rubric is shown in the following JSON string: \{rubric description\} \\

Please generate a score between 0 to 100 based on the given grading rubric (criteria) to indicate how good and suitable the code solution matches the request. \\

You can have the explanation, reasoning or analysis, but please explicitly generate the score using the format **Score: **, e.g., **Score: 37** in your response.
    

}
\end{tcolorbox}
\end{figure*}

==> tables/generalize_to_models.tex <==

\begin{table*}[htbp]
\centering
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{@{}lcccccc@{}}
\toprule
\textbf{Base Model} & \textbf{Agents} & \textbf{SR} & \textbf{VER} & \textbf{Cost} $\downarrow$ \\ 
 \midrule
\multirow{2}{*}{Claude-3.7} & Self-Debug & 22.5 & 84.3 & 0.066\\ 
 & \texttt{SciNav} (Ours) & \textbf{25.5} & 72.5 & 0.893\\
\midrule
\multirow{2}{*}{DeepSeek-R1} & Self-Debug &  18.6  & 59.8 & 0.023  \\ 
 & \texttt{SciNav} (Ours) & \textbf{19.6} & \textbf{67.6} & 0.298\\
\bottomrule
\end{tabular}
}
\caption{Generalization of \texttt{SciNav} to other base models. Mean performances of each agent on ScienceAgentBench \citep{chen2025scienceagentbench}. Among the reported metrics, SR (Success Rate) is the most important as it directly reflects task success. VER (Valid Execution Rate) indicates whether a program can be executed without errors and is closely related to the number of debugging steps. Note that we run \texttt{SciNav} with 3 debug steps, while Self-Debug is run with 10 debug steps, which may occasionally allow Self-Debug to achieve higher VER than \texttt{SciNav}.}
\label{tab:generalize_to_models}
\end{table*}


